Auction Design for Value Maximizers with Budget and Return-on-spend Constraints

The paper designs revenue-maximizing auction mechanisms for agents who aim to maximize their total obtained values rather than the classical quasi-linear utilities. Several models have been proposed to capture the behaviors of such agents in the literature. In the paper, we consider the model where agents are subject to budget and return-on-spend constraints. The budget constraint of an agent limits the maximum payment she can afford, while the return-on-spend constraint means that the ratio of the total obtained value (return) to the total payment (spend) cannot be lower than the targeted bar set by the agent. The problem was first coined by [Balseiro et al., EC 2022]. In their work, only Bayesian mechanisms were considered. We initiate the study of the problem in the worst-case model and compare the revenue of our mechanisms to an offline optimal solution, the most ambitious benchmark. The paper distinguishes two main auction settings based on the accessibility of agents' information: fully private and partially private. In the fully private setting, an agent's valuation, budget, and target bar are all private. We show that if agents are unit-demand, constant approximation mechanisms can be obtained; while for additive agents, there exists a mechanism that achieves a constant approximation ratio under a large market assumption. The partially private setting is the setting considered in the previous work [Balseiro et al., EC 2022] where only the agents' target bars are private. We show that in this setting, the approximation ratio of the single-item auction can be further improved, and a $\Omega(1/\sqrt{n})$-approximation mechanism can be derived for additive agents.

==> 20-preliminaries.tex <==
\subsection{Problem Fomulation}
\label{sec:pre}

The formal description of the auction environment is the following. 
One auctioneer wants to distribute $m$ heterogeneous divisible items among $n$ agents. 
Without loss of generality, assume that each item is of one unit since the items are \emph{divisible}. 
Each agent $i\in [n]$ has a value $v_{ij} $ for each item $j\in [m]$ and a budget $B_i $, representing the maximum amount of money agent $i$ can pay. 
The agent also has a target ratio $\tau^*_i$, representing the minimum ratio of the received value (return) to the total payment (spend) that she can tolerate. 
Per the literature convention, we refer to this constraint as the return-on-spend (RoS) constraint. 
As mentioned above, several settings of the type (public or private) of $\left( \vB,\vecv,\vtau \right)$ are considered in the paper. 
Agents are value maximizers subject to their budget constraints and RoS constraints. 
More specifically, if agent $i$ receives items with a total value of $v_i$ and pays $p_i$, the utility is stated in \cref{equ:utility}.
% \begin{equation}
% u_i:= \left\{
% 	\begin{aligned}
% 	v_i \;\;\;\;& \text{if $p_i\leq B_i$ and $p_i\tau_i \leq v_i$ }&  \\
% 	-\infty\;\;\;\; & \text{otherwise.}& \\
% 	\end{aligned}
% 	\right.
% \end{equation}
The auctioneer aims to design a truthful mechanism that maximizes the total payment, i.e., $\sum_{i\in[n]}p_i$.
%\ruilong{may need to mention the definition of truthfulness and approximation ratio}
\iffalse
In this paper, we will leverage the following lemma stated in~\cite{DBLP:conf/sigecom/BalseiroDMMZ22} to prove the truthfulness of the proposed mechanisms. Let $\vtau$ and $\vtau_{-i}$, respectively, be the target ratio profiles of all the agents and all the agents except $i$. For an agent $i$, use $U_i(\vtau)$ and $P_i(\vtau)$ to denote her received value and payment respectively if the reported target ratio profile is $\vtau$.
\chenyang{To Do}
\begin{lemma}[\cite{DBLP:conf/sigecom/BalseiroDMMZ22}]\label{lem:truthful}
    A mechanism is truthful if and only if it is feasible and for every agent $i$ and any $\vtau_{-i}$,
    \begin{itemize}
        \item [(1)]
        $U_i(\tau_i,\vtau_{-i})$ is non-increasing as $\tau_i$ increases;
        \item [(2)]
        For any $\htau_i < \tau_i$, if $U_i(\htau_i,\vtau_{-i})>U_i(\tau_i,\vtau_{-i})$, then $U_i(\htau_i,\vtau_{-i}) < \tau_i P_i(\htau_i,\vtau_{-i})$.
    \end{itemize}
\end{lemma}

On an intuitive level, condition (1) in the lemma prevents an agent from misreporting a target ratio higher than the actual ratio since the agent is a value maximizer, while condition (2) guarantees that the agent cannot misreport a ratio lower than the actual ratio because otherwise, her RoS constraint will be violated.

\begin{itemize}
    \item definition
    \item useful lemmas in the previous paper
\end{itemize}

\fi
